Asynchronous rotation of Earth-mass planets in the habitable zone of lower-mass stars

Planets in the habitable zone of lower-mass stars are often assumed to be in a state of tidally synchronized rotation, which would considerably affect their putative habitability. Although thermal tides cause Venus to rotate retrogradely, simple scaling arguments tend to attribute this peculiarity to the massive Venusian atmosphere. Using a global climate model, we show that even a relatively thin atmosphere can drive terrestrial planets' rotation away from synchronicity. We derive a more realistic atmospheric tide model that predicts four asynchronous equilibrium spin states, two being stable, when the amplitude of the thermal tide exceeds a threshold that is met for habitable Earth-like planets with a 1-bar atmosphere around stars more massive than 0.5-0.7Msun. Thus, many recently discovered terrestrial planets could exhibit asynchronous spin-orbit rotation, even with a thin atmosphere.

==> referee.tex <==
Referee:

- Jacques Laskar
laskar@imcce.fr
Department "Astronomie et Systèmes Dynamiques", IMCCE, Observatoire de Paris 

- Alexandre Correia
correia@ua.pt
Department of Physics, University of Aveiro, Portugal

- Piet Hut
piet@ias.edu
Institute for Advanced Study, Princeton

- Andrew Ingersoll
api@gps.caltech.edu
Caltech Division of Geological and Planetary Sciences, California

- Anthony Dobrovolkis
anthony.r.dobrovolskis@nasa.gov
SETI Institute, NASA Ames Research Center Moffett Field, California


- James Kasting
kasting@essc.psu.edu
Department of Geosciences, The Pennsylvania State University, University Park, PA 16801

